Study of hard double-parton scattering in four-jet events in $pp$ collisions at $\sqrt{s} = 7$ TeV with the ATLAS experiment

Inclusive four-jet events produced in proton-proton collisions at a centre-of-mass energy of $\sqrt{s} = 7$ TeV are analysed for the presence of hard double-parton scattering using data corresponding to an integrated luminosity of 37.3 pb$^{-1}$, collected with the ATLAS detector at the LHC. The contribution of hard double-parton scattering to the production of four-jet events is extracted using an artificial neural network, assuming that hard double-parton scattering can be approximated by an uncorrelated overlaying of dijet events. For events containing at least four jets with transverse momentum $p_{\mathrm{T}} \geq 20$ GeV and pseudorapidity $\eta \leq 4.4$, and at least one having $p_{\mathrm{T}} \geq 42.5$ GeV, the contribution of hard double-parton scattering is estimated to be $f_{\mathrm{DPS}} = 0.092 ^{+0.005}_{-0.011} (\mathrm{stat.}) ^{+0.033}_{-0.037} (\mathrm{syst.})$. After combining this measurement with those of the inclusive dijet and four-jet cross-sections in the appropriate phase space regions, the effective overlap area between the interacting protons, $\sigma_{\mathrm{eff}}$, was determined to be $\sigma_{\mathrm{eff}} = 14.9 ^{+1.2}_{-1.0} (\mathrm{stat.}) ^{+5.1}_{-3.8} (\mathrm{syst.})$ mb. This result is consistent within the quoted uncertainties with previous measurements of $\sigma_{\mathrm{eff}}$, performed at centre-of-mass energies between 63 GeV and 8 TeV using various final states, and it corresponds to $21^{+7}_{-6}$% of the total inelastic cross-section measured at $\sqrt{s} = 7$ TeV. The distributions of the observables sensitive to the contribution of hard double-parton scattering, corrected for detector effects, are also provided.

==> colors.tex <==
\definecolor{myRootCol0}{rgb}{0.2,0.2,0.2}
\definecolor{myRootCol1}{rgb}{1.0,0.4,0.4}
\definecolor{myRootCol2}{rgb}{0.2,0.4,0.8}
\definecolor{myRootCol3}{rgb}{1.0,0.6,0.0}
\definecolor{myRootCol4}{rgb}{0.4,0.6,0.0}
\definecolor{myRootCol5}{rgb}{0.0,0.0,0.4}
\definecolor{myRootCol6}{rgb}{1.0,0.2,1.0}
\definecolor{myRootCol7}{rgb}{0.0,0.8,0.2}
\definecolor{myRootCol8}{rgb}{0.6,0.4,0.2}
\definecolor{myRootCol9}{rgb}{0.0,0.6,0.6}
\definecolor{myRootCol10}{rgb}{1.0,0.0,0.0}
\definecolor{myRootCol11}{rgb}{0.6,0.6,0.6}
\definecolor{myRootCol12}{rgb}{0.2,0.2,0.4}
\definecolor{myRootCol13}{rgb}{0.8,0.4,1.0}
\definecolor{myRootCol14}{rgb}{0.2,0.6,0.0}
\definecolor{myRootCol15}{rgb}{0.6,0.0,0.0}
\definecolor{myRootCol16}{rgb}{0.8,0.0,0.8}
\definecolor{myRootCol17}{rgb}{1.0,0.2,0.4}
\definecolor{myRootCol18}{rgb}{0.6,0.4,1.0}
\definecolor{myRootCol19}{rgb}{0.4,0.4,0.2}

